Unsupervised Discovery of 3D Physical Objects from Video

We study the problem of unsupervised physical object discovery. While existing frameworks aim to decompose scenes into 2D segments based off each object's appearance, we explore how physics, especially object interactions, facilitates disentangling of 3D geometry and position of objects from video, in an unsupervised manner. Drawing inspiration from developmental psychology, our Physical Object Discovery Network (POD-Net) uses both multi-scale pixel cues and physical motion cues to accurately segment observable and partially occluded objects of varying sizes, and infer properties of those objects. Our model reliably segments objects on both synthetic and real scenes. The discovered object properties can also be used to reason about physical events.

==> figText/cubes_qualitative.tex <==
\begin{figure}[t]
\centering
% \begin{wrapfigure}{l}{0.5\textwidth}
% \vspace{-6mm} 
\includegraphics[width=.8\linewidth]{fig/qual_pred_block.pdf}
\caption{Qualitative comparisons of unsupervised object segmentation of \model with and without physics and with MONet on realistic block towers. MONet often groups two blocks together when having similar color (dark blue/green) and sometimes misses particular blocks. \model with multiscale architecture is able to reliably detect all blocks, but still often group blocks that look similar (dark blue/green) into one block. \model with multiscale and physical consistency is able to reliably detect all objects and assign different masks to each object. \jw{The gaps between neighboring columns are too large. Also images in the same row are not horizontally aligned...}} 
\label{fig:cubes_qualitative}
\end{figure}

==> figText/iou_cubes.tex <==
\begin{table}[t]
\small
\caption{Average IoU segmentation results on the real blocks data set, as well as the percentage of objects that are detected, where at least one segmentation mask has greater than 0.5 IoU. \jw{We may consider merging Table 3 with Figure 7 (qualitative results on blocks).  Also add confidence intervals.}}
\label{tbl:iou_block}
\begin{center}
\begin{tabular}{l|cccc}
% \multicolumn{1}{c}{\bf Color}  &\multicolumn{1}{c}{\bf DESCRIPTION}
\toprule
\bf Model & \bf Multi-Scale & \bf Phys & \bf IoU & \bf Detection (\%) \\ 
\midrule
MONET & - & - & 0.521 & 0.537 \\
OP3 & - & - & 0.311 & 0.250 \\
\midrule
\model & No & No & 0.546 & 0.523 \\
\model & Yes & No & 0.746  &  0.785 \\    
\model & Yes & Yes & \textbf{0.822} & \textbf{0.914}\\    
\bottomrule
\end{tabular}
\end{center}
\end{table}

==> figText/motion_generalize.tex <==
% \begin{table}[t]
% \small
% \caption{Comparison of generalization of \model with or without physical constancy, measured in average IoUs on segmentation, and in the percentage of objects that are detected. %, where at least one segmentation mask has greater than 0.5 IoU. 
% Including physics integrates the motion signal and generalizes better to both datasets of novel shapes and novel patterns.}
% \label{tbl:iou_adept_generalize}
% \begin{center}
% \begin{tabular}{lcccc}
% % \multicolumn{1}{c}{\bf Color}  &\multicolumn{1}{c}{\bf DESCRIPTION}
% \toprule
% \bf Generalization & \bf Model &  \bf Phys & \bf IoU & \bf{Detection (\%)} \\ 
% \midrule
%  \multirow{2}{*}{Shape} & \model & No & 0.768  &  0.823 \\    
%  & \model & Yes &  0.857 & 0.922 \\    
% \midrule
% \multirow{2}{*}{Texture} & \model & No & 0.658  &  0.716 \\    
% & \model & Yes &  0.756 & 0.843\\    
% \bottomrule
% \end{tabular}
% \end{center}
% \end{table}

==> text/broader_impacts.tex <==
\section*{Broader Impact}
Our work is a step towards the broad goal of building a system with  physical understanding of the scenes around it. A system with a broad physical understanding of its surrounding environment has many potential impacts in industrial domains such as enabling household robots that can help the elderly age in place by helping with household chores and monitoring medical treatment. On the other hand, errors in our scene understanding system, such as classifying an unstable multi-object structure as a single object, could be costly if the model were actually deployed. We do not foresee our model, as a preliminary research effort, to have any significant societal impact toward any particular group.
